Quantum-enhanced absorption spectroscopy with bright squeezed frequency combs

Absorption spectroscopy is a widely used technique that permits the detection and characterization of gas species at low concentrations. We propose a sensing strategy combining the advantages of frequency modulation spectroscopy with the reduced noise properties accessible by squeezing the probe state. A homodyne detection scheme allows the simultaneous measurement of the absorption at multiple frequencies and is robust against dispersion across the absorption profile. We predict a significant enhancement of the signal-to-noise ratio that scales exponentially with the squeezing factor. An order of magnitude improvement beyond the standard quantum limit is possible with state-of-the-art squeezing levels facilitating high precision gas sensing.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
